jpf-concurrent: An extension of Java PathFinder for java.util.concurrent

One of the main challenges when verifying multi-threaded Java applications is the state space explosion problem. Due to thread interleavings, the number of states that the model checker has to verify can grow rapidly and impede the feasibility of verification. In the Java language, the source of thread interleavings can be the system under test as well as the Java Development Kit (JDK) itself. In our paper, we propose a method to minimize the state space explosion problem for applications verified under the Java PathFinder (JPF) model checker. Our method is based on abstracting the state of the application to a smaller domain and implementing application behavior using the Model Java Interface (MJI) of JPF. To show the capabilities of our approach, we have created a JPF extension called jpf-concurrent which abstracts classes from the Java Concurrency Utilities. Several benchmarks proved the usefulness of our approach. In all cases, our implementation was faster than the JDK implementation when running under the JPF model checker. Moreover, our implementation led to significantly smaller state spaces.

==> ack.tex <==
\section*{Acknowledgement}
The authors would like to thank Dave Parker, Franck van Breugel and anonymous reviewers for their invaluable comments.
A special acknowledgement goes to Peter Mehlitz for his constant support during whole development
of jpf-concurrent. In 2008 and 2011 development of this project has been funded by Google as a part of Google Summer of Code program.

==> benchmarks.tex <==
\section{Benchmarks}
All benchmarks have been performed on a Dell PowerEdge R410 machine, with 32GB of RAM, 6 Xeon processors
running Fedora 14. Each run has been repeated 10 times. Three classes have been used for benchmarking, {\tt ReentrantLockPerformanceTest}, 
{\tt ConcurrentHashMapPerformanceTest}, and {\tt AtomicIntegerPerformanceTest}. All of these classes can 
be found in the jpf-concurrent website \footnote{http://babelfish.arc.nasa.gov/trac/jpf/wiki/projects/jpf-concurrent}. Results have been summarized in Table I.

We have used these classes to show the most prominent types of concurrency constructs 
that can be found in Java Concurrency Utilities. {\tt ReentrantLock} represents
classes that heavily depend on thread blocking instructions. {\tt ConcurrentHashMap} is an example of a
data structure that tries to avoid thread blocking in all feasible cases.
Finally, {\tt AtomicInteger} represents all classes that use CAS operations \cite{wait-free}
to achieve atomicity of instructions.

In all cases, jpf-concurrent shows a speedup. The speedup for the {\tt ReentrantLock} 
is much higher than for {\tt ConcurrentHashMap} and {\tt AtomicInteger}. 
This is caused by the fact that using native methods allows us to use fewer thread-blocking
operations which are the main source of new transitions, and that can increase the verification time. The smallest speedup
has been obtained for {\tt AtomicInteger}, CAS operations are by definition
atomic, therefore, moving implementation to native methods did not affect the state space significantly.
Due to the exponential increase in test time we were not able to obtain results for a number 
of threads higher than 6 and 12. Despite this fact, even for small numbers of threads we 
can see a trend where speedup grows with the number of threads. 

In all cases memory consumption has been a little bit smaller for code run under jpf-concurrent.
We attribute this to simplification of data structures that are used on host VM level. Since the difference has been almost negligible, memory usage is not included in the Table I.
When used with {\tt ObjectRemovalListener}, our method can produce a significant memory overhead. In the presence of backtracking objects that has been garbage collected on one execution path might be still used on the others.
To handle such a situation we need to keep additional information regarding execution paths and monitored objects which results in increased memory usage. Said that, to this point we have not encountered a real life example that would require {\tt ObjectRemovalListener}. 


One publicly known case where jpf-concurrent has been used to help verify large NASA applications is \cite{jpf_awt:pub}, but there motivation is support for unimplemented native methods, rather than improved performance.

==> conclusions.tex <==
\section{Conclusions}

In this paper we proposed a new technique to model Java Concurrency Utilities within JPF. 
%Applying our approach leads to a considerably smaller state space and reduces verification time.
We implemented an extension to JPF called jpf-concurrent which is based on the proposed approach. 
Our approach not only reduces the state space of the program but also provides support 
for native calls within the Java Concurrency Utilities that have not been supported in the JPF core project.
 
Using a set of benchmarks, we have shown that in all cases jpf-concurrent provides a speedup for different types
of classes included in Java Concurrency Utilities. At the time of writing this paper
the jpf-concurrent project has been actively developed for more than three years, and it is considered one of the most
popular extensions of the JPF model checker.

In the future we plan to extend jpf-concurrent to support all classes included in the 
Java Concurrency Utilities, including new constructs that have been 
introduced within Java 6 and 7. Another future direction includes supporting operations that 
rely on time. At this point JPF uses system time which in the presence of 
backtracking is no longer valid and can lead to bugs that are extremely hard to debug. 
We also think that researching new methods used for state matching within jpf-concurrent can lead to a significant
reduction of the verification time and should be considered in the future.


==> intro.tex <==
\section{Introduction}
The state space explosion problem is known as one of the most challenging issues in model checking \cite{book:mch,book:pmch}. 
One of the sources of this problem is thread non-determinism. In programs that include thread 
non-determinism, the concurrent actions can be executed in any order. In such programs, 
considering all possible interleavings of these concurrent actions can lead to a very large 
state space that cannot be stored in the available memory resources or processed in 
reasonable time. It can be shown that the number of program states 
can increase exponentially with the number of concurrently running components  \cite{book:pmch}.

% JPF

Java PathFinder (JPF) \cite{Brat-al:AV00} is an explicit-state model checker that directly works with Java bytecode instructions.
The core of JPF is a Java Virtual Machine (JVM) which systematically executes Java programs by
exploring all possible thread interleavings. Each execution is a sequence of transitions and each 
transition is a sequence of bytecode instructions that takes the system from one state to another. 
While JPF is executing the program, it explores the program state space. JPF, as any other model checker, suffers from the state space explosion problem.

% JPF and state space explosion from JDK code
% we need to say about perfomance + Unsafe problems.

Java applications use the JDK to simplify the development process. For concurrent applications the JDK provides Concurrency Utilities ({\tt java.util.concurrent} package) which contains implementations of basic concurrency constructs. As JPF is mostly used to verify multi-threaded code, a large number of applications verified under JPF use classes from Java Concurrency Utilities. 
%%
Verifying Java programs which are based on Java Concurrency Utilities gives rise to several challenges.
In general, due to thread non-determinism originated from many constructs included in Java Concurrency Utilities, model checking such Java programs leads to very large state spaces. 
Another challenge is compatibility issues between different JRE/JDK vendors. To improve performance a large number of vendors use private classes to implement {\tt java.util.concurrent} package. These classes tend to contain native methods, the implementation of which is tied to a specific JVM. To run such code JPF would have to handle these native methods for each JVM vendor. This has not been done, and in many cases running code that uses  classes from Java Concurrency Utilities triggers an {\tt UnsatisfiedLinkError} error. 
%Last observed problem were unreadable stack traces due to size of the Java Concurrency Utilities and a number of method calls that were kept on the stack.
Finally, unreadable stack traces is another issue which is due to the size of the Java Concurrency Utilities and the number of method calls that are kept on the stack.

%Briefly state our solution
To solve the above issues, we have created the jpf-concurrent extension for JPF. In this extension, model classes are created as replacements for the classes included in the Java Concurrency Utilities. The size of the state space is reduced by abstracting the state of the Java Concurrency Utilities classes to a single integer declared within their corresponding model classes. Moreover, the MJI feature of JPF is used to delegate most of the implementation of concurrent classes to the host JVM level where it is not model checked. Using this technique, we keep the complex state of the concurrent objects on the host JVM, and JPF uses an integer to represent different states. Native method compatibility problems have been solved by reimplementing most of the Java Concurrency Utilities classes without using any vendor specific code. Our solution also shortened the size of the stack traces considerably.

The rest of this paper is organized as follows. In Section II we discuss related work and existing solutions. Section III presents an example of how jpf-concurrent can be used for software verification. In Section IV the reader can find detailed description of jpf-concurrent implementation.  Section V contains quantitative results of running the benchmarks. Finally, we outline future work in Section VI.



==> related_work.tex <==
\section{Related Work}
There exist several programming interfaces within JPF that can be used to solve the presented issues.
To provide implementation for unsupported native methods and reduce the state space JPF contains Model Java Interface (MJI). In resemblance to Java Native Interface (JNI), which is used to transfer the execution from the Java level to the native level, MJI is used to transfer the execution from JPF to the host JVM. All methods that execute on the host JVM using MJI are atomic, therefore, they do not 
contribute to the state space explosion problem.
In the cases where a method has to be executed on the JPF level, in order to avoid thread reschedulings, we can use the
class {\tt gov\.nasa\.jpf\.jvm\.Verify}. This class includes the methods {\tt beginAtomic()} and {\tt endAtomic()}. All the bytecode instructions surrounded by these two methods are combined into a single transition. 
Reducing the stack traces can be achieved by means of a listener. Such a listener could extend the {\tt ListenerAdapter} class and implement the {\tt propertyViolated()} method to access and augment the current stack trace.
To the best of our knowledge, before jpf-concurrent there was no work that would provide a coherent usage of these techniques
that would allow state abstraction on the JPF level and state handling on the host VM level.
There are a few other JPF extensions that reimplement JDK libraries to allow verification. jpf-awt \cite{jpf_awt:pub}
focuses on AWT/Swing libraries and uses MJI to reimplement {\tt EventDispatchThread} where it reads UI scripts that are used as drivers for the verification process. Another extension is net-iocache \cite{net_iocache:pub, net_iocache:pub2} which allows verification of networking applications in the presence of backtracking. 
Unfortunately, because of unique characteristics of GUI and networking applications none of these techniques can be directly applied to Java Concurrency Utilities.  
%here (or before mentioning other extensions) we need say that none of the work perfectly fits our need
%MJI and Verify exists but there was no systematic way to abstract and keep state on host VM level
%the idea is that the reader after this sections needs to have an idea how our work is different from previous work


%Our approach is based on these two techniques, and it leads to a much smaller state 
%space while preserving the same behaviour of modeled code. We also abstract the state of objects 
%into a smaller domain which effectively reduces the verification time. To prove the usefulness of our approach
%we have created the jpf-concurrent project which is an extension to JPF. 
%jpf-concurrent provides a model for Java Concurrency Utilities \cite{jsr166:URL}. It replaces
%classes included in the {\tt java.util.concurrent} package with the optimized versions. 
%Moreover, jpf-concurrent provides support for the 
%native calls that were not handled within JPF increasing the spectrum of applications
%that can be verified. Our extension also gets rid of any dependency to the 
{%\tt sun\.misc\.Unsafe} class in the {\tt java.util.concurrent} package.
%This class is not part of the JSR 166 specification, and it is a private 
%implementation of one of the JVM vendors which lead to vendor specific code that had to be
%included in JPF.
%Finally, jpf-concurrent reduces the size of the stack traces making debugging of multi-threaded 
%code easier.

% reasons to model Java concurrency utilities
%Though our method can be applied to any code verified under JPF, we choose to model the Java Concurrency Utilities among other %Java standard libraries. One reason that we chose to model this library is the fact that concurrency is becoming more and more %important as machines get more and more cores \cite{microproc}. Java Concurrency Utilities are extensively used by programmers %to create multi-threaded Java applications. Since it is notoriously hard to detect errors in these systems, any tools that can assist %programmers to detect bugs in their code are very useful. 
%Another reason for choosing Java Concurrency Utilities is reducing the state space and improving the verification time for code %based on this particular library. Due to thread non-determinism, model checking code which is based on Java Concurrency Utilities %gives rise to very large state space. 
